CoRE: Condition-based Reasoning for Identifying Outcome Variance in Complex Events

Knowing which latent conditions lead to a particular outcome is useful for critically examining claims made about complex event outcomes. Identifying implied conditions and examining their influence on an outcome is challenging. We handle this by combining and augmenting annotations from two existing datasets consisting of goals and states, and explore the influence of conditions through our research questions and Condition-based Reasoning tasks. We examine open and closed LLMs of varying sizes and intent-alignment on our reasoning tasks and find that conditions are useful when not all context is available. Models differ widely in their ability to generate and identify outcome-variant conditions which affects their performance on outcome validation when conditions are used to replace missing context. Larger models like GPT-4o, are more cautious in such less constrained situations.

==> acl_templ.tex <==
\begin{abstract}
This document is a supplement to the general instructions for *ACL authors. It contains instructions for using the \LaTeX{} style files for ACL conferences. 
The document itself conforms to its own specifications, and is therefore an example of what your manuscript should look like.
These instructions should be used both for papers submitted for review and for final versions of accepted papers.
\end{abstract}

\section{Introduction}

These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,borschinger-johnson-2011-particle,andrew2007scalable,rasooli-tetrault-2015,goodman-etal-2016-noise,harper-2014-learning}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliographystyle{acl_natbib}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> sections/acknowledgements.tex <==
%\section{Acknowledgments}
We would like to thank the anonymous reviewers for their comments, questions, and suggestions. We would also like to thank Katrin Erk, Sayontan Ghosh and Niranjan Balasubramian for early discussions and
feedback. This material is based in part upon work supported by the National Science Foundation under Grant No. IIS-2024878. Some experiments were conducted on the UMBC HPCF, supported
by the National Science Foundation under Grant No. CNS-1920079. This material is also based on research that is in part supported by the Army Research Laboratory, Grant No. W911NF2120076,
and by the Air Force Research Laboratory (AFRL), DARPA, for the KAIROS program under agreement number FA8750-19-2-1003. The U.S. Government is authorized to reproduce and distribute
reprints for Governmental purposes notwithstanding any copyright notation thereon. The views and
conclusions contained herein are those of the authors and should not be interpreted as necessarily representing the official policies or endorsements, either express or implied, of the Air Force Research
Laboratory (AFRL), DARPA, or the U.S. Government.

==> sections/augmentation.tex <==
\section{Data Augmentation}
\label{sec:dataset}

We made the following augmentations to SAGA and PASTA annotations to explore conditions and outcomes:

\begin{enumerate}[(1)] 
\item We rewrote the SAGA goal descriptions as ongoing and completed actions using GPT-3.5-Turbo.  SAGA goals are not always grammatically correct and complete sentences;  we wrote 3 seed examples (without using any story context) and using these rewrote 100 SAGA goals from the training data split as complete  grammatical sentences describing completed actions.  The authors manually verified that the generated claims are grammatically correct and complete sentences reflecting a completed goal relevant to the story.  Using the verified examples we rewrote the remaining goals and manually verified using the same checks as with the first 100.
\item Asking whether the outcomes (both ongoing and completed actions) from the above step can be inferred from the story context (using both actual and alternate story contexts of SAGA), we manually annotated whether each outcome is true, false or unsure for the given story.  We computed agreement with the crowd annotations in the next step to show that these manual annotations are in fairly good agreement with the crowd annotations.   
\item The goal achievement annotation in SAGA based on 5-point likert scale from Unsuccessful to Fully Successful is not always accurate.  We used the goal achievement evaluation scores from the 3 crowd workers for the test and validation data splits to automatically correct the achievement annotation %(we examined and made minor manual corrections for unsure achievement values which could not be automatically corrected since the unsure value could have been used for multiple reasons).  
\item We convert the 5-point likert scale to the 3 outcome labels of True/False/Unsure (Fully \& Moderately Successful labels are converted to an outcome label of true and Less \& Un- Successful labels are converted to an outcome label of false). We compute IAA between our outcome label annotations and these automatically corrected crowd annotations and achieve a Cohen's Kappa score of .64 (without the corrections this score is .54). A majority of disagreement is due to unsure labels and if we were to consider only the true and false labels the IAA is .73 (without the corrections this score is .63) showing that our claim label annotations are in good agreement  with the crowd, especially after applying corrections based on multiple worker evaluations. 
\item Each of the 5 sentences in a SAGA actual story was assigned one of 6 labels to identify the relation between the event in the sentence and the goal by a crowd worker.  We map these 3 relation labels as follows to identify the relationship between the sentence and outcome: any goal justifying and enabling relations are labeled \textit{Support}, any goal blocking relation is labeled \textit{Oppose} and the remaining are labeled \textit{No-Effect}.  We realize this mapping can be noisy, especially for data in the training split which could not be corrected in the above step (the evaluation scores were only available for test and validation data splits).  Using the SAGA sentence relations we automatically identify one of the 3 above relations for each condition (using the PASTA sentence annotations that identify which sentences a condition is based upon).  We assume the counterfactual condition would have the opposite relation which can be noisy.  These relations identify how a condition relates to the outcome (aka outcome-oriented relation annotations).
\item  We automatically identify if a condition and its contrastive condition are outcome- variant, invariant or unsure using the claim label annotations from the two stories and our definitions in \cref{sec:conditions-outcomes}.
\item  We use Spacy to obtain the root verb of PASTA states (aka conditions) and categorize these descriptions into stative and action-oriented expressions to identify the lexical type of the annotation.  About a third are activity oriented expressions and two-thirds are stative expressions. We also categorize the conditions using the 4 categories from \cref{sec:conditions-outcomes}. 
\item  We obtain a random 125 news stories from the POQUE dataset~\cite{vallurupalli-etal-2022-poque} and obtain SAGA-style goal descriptions and their achievement success annotation using crowd-workers on Amazon Mechanical Turk.  Workers were paid \$.40 per story.  We also obtained goal descriptions using GPT3.5 to compare with the crowd-annotated goals.    We had 3 workers evaluate to ensure both crowd and model annotated goal annotations and are valid and paid \$.10 per each goal evaluation for the the 250 goal annotations.  We followed the same process as in steps 1 and 2 above to obtain an outcome and its truth label.  
\end{enumerate}


 













\begin{table}[t]
\centering
\resizebox{.98\columnwidth}{!}{
\small
\begin{tabular}[trim=0 .2in 0 0,  width=.98\linewidth]{p{0.48\linewidth} | p{0.48\linewidth}  }
\hline\hline
Annotation  &   Augmented SAGA/PASTA   \\ 
\hline\hline
Story Contexts & 886 (Actual) / 951 (Alternate) \\
\hline
Claims &  2985  \\
\# Condition Pairs  &  951 \\
\# Condition applied to Claim   & 6989\\
\hline
Claim Labels & 2125 / 299 / 561  \\ 
(identify claim truthfulness)&(True/False/Unknown) \\ 
%Test Progressive (708/305/118) Perfect (609/399/123) 
\hline
Corrected Goal Labels  & 2125 / 484 / 376 \\
(identify goal achievement)&(Success/Unsuccess/Unsure) \\
\hline
Event-Goal Relations & 13140 / 1230 / 555 \\  
(5 relations per claim)& (Support/Oppose/No-Effect) \\ \hline
Condition Type & 6607 / 3448 / 3923\\ 
(condition-outcome relation)& (Support/Oppose/No-Effect)\\
%\hline
%Condition Category & \\
\hline
Outcome-oriented Relations & 1985   / 694   / 598  \\
(a condition-pair's relation)& (variant/invariant/unsure)\\
\hline
\hline
\end{tabular}
}
\caption{ Data Statistics for the augmented SAGA \& PASTA dataset.  }
\label{tab:annotation-details}
\vspace{-5mm}
\end{table}

 

==> sections/cutouts.tex <==
\textbf{Actual Story:}
1. Jimmy went canoeing with his best friend Carl.
2. Jimmy's mother told him to wear a life vest.
3. Jimmy ignored her advice, and didn't wear one.
4. Jimmy fell out of the boat, and almost drowned.
5. From then on, Jimmy listened to his mother.
\end{quote}
 \begin{figure}
    \centering     \includegraphics[trim=0 .2in 0 0,  width=.9\textwidth]
    {sections/figures/goal-state_fig_v1.png}
    \vspace{-35mm}
	\caption{A Change in a participant's state leads to a counterfactual story situation changing the participant's and other participants' goal achievement. %
 }
	\label{fig:fig1}
 \vspace{-5mm}
\end{figure}
We can infer that Jimmy's goal is ``to go canoeing without any incidents.'' Consider the alternate situation below (a counterfactual story from PASTA~\cite{ghosh2023pasta}) where Jimmy's goal is unchanged, albeit, with a slightly different set of actions.   

\begin{quote} 
\small
\textbf{Counterfactual Story:}
1. Jimmy went canoeing with his best friend Carl.
2. Jimmy's mother told him to wear a life vest.
3. Jimmy ignored her advice, and didn't wear one.
4. Jimmy fell out of the boat, and almost drowned.
5. Jimmy continued to go without a life vest.

\end{quote}
From this counterfactual story we understand the implied state that Jimmy did not learn from his previous fall.  While this state did not affect the participant's goal, if the last sentence was As illustrated in \cref{fig:fig1}, the state change affects the goal achievement of the participant in this counterfactual story.
In the counterfactual Jimmy may not achieve his goal which can affect his mother's goal achievement of "wanting her son's safety".  Knowledge of goals and the conditions that influence them can help a participant revise their plan to change their achievement.  For example, noticing that the currents are rapid Jimmy can wear an emergency life vest on his canoe.   


%\paragraph{Coherence:}  Measures how many of the participant's actions in the story are covered by the goal.   High coherence indicates that all actions are aimed at achieving the described goal.   Low coherence indicates only some of the actions are aimed at achieving the goal.%\paragraph{Explain-abiliy Coverage:} Measures how much of the goal can be explained by the participant's actions.  High coverage indicates the goal can be fully explained by the actions. Low coverage indicate the goal cannot be fully explained by the actions.%\paragraph{Means-end Clarity:} Measures whether the goal description asserts a clear and rational means-end belief explanation of the participant's intention. High clarity indicates a clear unconditional goal that the participant believes can be achieved~\cite{Grice1971-GRIIAU} regardless of the actual outcome.  




%\subsection{Goal Parameters}
%From the story context we can identify the goal dimensions relating to content and intensity:  the difficulty of the goal, a participant's commitment, influence from external factors, state of success, whether the participant would consider a revision and the participant's satisfaction.  Thus we collect the following goal dimensions for each super-ordinate goal: 

%\paragraph{Goal Difficulty $GD_i$:}
%The story context give an indication of the participant's thoughts on the difficulty of achieving their goal.  If this information cannot be inferred from the story, this value is based on an annotator's external knowledge about how difficult the abstract goal achievement will be.  \textit{Possible values of $GD_i$ are: Very Easy, Somewhat Easy, Unsure, Somewhat Difficult, Very Difficult}.

%\paragraph{Goal Commitment $GC_i$:}
%The story context indicates how committed the participant is to achieving their goal.  If this information cannot be inferred from the story, this value is based on an annotator's external knowledge of the commitment required for achieving the abstract goal.  \textit{Possible values of $GC_i$ are: Very High, Somewhat High, Unsure, Somewhat Low, Very Low}.

%\paragraph{Goal Cooperation $GCP_i$:}
%Story events not in the participant's control could assist or hinder the achievement of a participant's goal.  The cooperation or conflict a participant experiences as inferred from the story events is captured by this value. \textit{Possible values of $GI_i$ are: Active Cooperation, Passive Cooperation, None, Passive Conflict, Active Conflict}.

%\paragraph{Goal Conflict $GCP_i$:}
%Story events not in the participant's control could assist or hinder the achievement of a participant's goal.  The cooperation or conflict a participant experiences as inferred from the story events is captured by this value. \textit{Possible values of $GI_i$ are: Active Cooperation, Passive Cooperation, None, Passive Conflict, Active Conflict}.

\paragraph{Goal-State pairs $G^p_i, PS^p_i$:}
Since we want to track the influence of a state change on goal achievement, using a second HIT, for each story $S^p(=S)$, we collect which goals of a participant are also applicable to the corresponding counterfactual stories and whether the goals are achieved in the story.  To measure \textit{presupposition bias}, we ask if the story makes sense and identify the sentences that lead to confusion.   

\paragraph{Goal Achievement based on State:}
For the goals that are not successful in the above HIT we use a third HIT and verify if the Next Action, $N_{ik}$ collected for assessing the goal $G^p$ (where $G^p$=$G_{ik}$) can be used for assessing goal direction in the counterfactual story.  When it can be used we denote it as $NA^p$, otherwise, we obtain a modified Next Action, $NA^{p'}$.  We also obtain annotations for Goal Success, $GS^{p'}_i$, Goal Direction, $GD^{p'}_i$, Goal Revision $GS^{p'}_i$ which apply to the counterfactual story, $S^{p'}$, using either the original or modified Next Action, $NA^p$ or $NA^{p'}$.  For the actual story $S^p$, we denote the Goal Success $GS_{ik}$ as $GS^p$, Goal Direction $GD_{ik}$ as $GD^p$ and Goal Revision $GR_{ik}$ as $GR^p$.  

%\subsection{Crowd Vs AI Annotations}
%\label{sec:Crowd_vs_AI}
%To decide whether to collect annotations from crowd workers on Amazon Mechanical Turk (AMT) or employ an AI model (specifically GPT3.5), we obtained 3 goal annotations from each of the two sources to explain a participant's actions in 250 stories (=6 annotations for a equal number of Newswire and ROC stories).  We designed a human intelligence task (HIT) for collecting crowd annotations and a prompt collecting GPT3.5 annotations for a participant's goal given a story in which the participant mentions are highlighted.  More on the HIT and prompts details are discussed in \cref{sec:HIT_Prompt}.
 
%We validated the collected annotations using the goal evaluation criteria in \cref{sec:Evaluation_Criteria} using 3 crowd workers.  We noticed that the nature of the stories and the task steps elicit a variation in the text style and format, even from the same worker. As expected crowd produced more nuanced goal annotations as shown in table ... when compared to model annotations~\cite{Holtzman2020The,Welleck2020Neural}.  Because model generated content could already contain and lead to misinterpreting reality based on reinforced beliefs~\cite{shumailov2023curse} we decided to obtain annotations from crowd workers. 

%In this initial collection we focused on annotations for a single participant in a story.   We prompted GPT3.5 (text-davinci-003) model to obtain the same 10 annotations. More on the prompts used and HIT details are discussed in \cref{sec:HIT_Prompt}

%Knowledge distillation~\cite{Model_compression,hinton2015distilling,west2022symbolic} has been shown to produce effective task-specific models using knowledge collected from a capable larger model. 
%Crowd workers improved the quality of symbolic knowledge collected from larger models ~\cite{Wiegreffe2021ReframingHC,liu2022wanli} reducing repetition~\cite{Geirhos_2020}, reporting~\cite{gordon2013reporting} and annotator~\cite{geva-etal-2019-modeling,gururangan-etal-2018-annotation}  biases. 
%Evaluating annotations from crowd workers and instruction finetuned language models FlanT5 (xxl-model) and GPT3.5 (text-davinci-003) ~\cite{wei2022finetuned,chung2022scaling,ouyang2022training}
%that are both  that perform well on reasoning in unseen tasks  
%we found  reinforcement learning from human feedback (RLHF)~\cite{ouyang2022training} is better at goal reasoning (discussed in \cref{sec:initial_annotations}).  We leverage the human likability of language scaffolding \cite{clark-etal-2021-thats} and use GPT3 generations as assists for crowd workers to produce more elaborate and nuanced annotations.  

\includegraphics[trim=0 .2in 0 0,  width=.95\linewidth]
     {sections/figures/goal-state_fig3_v2.png}
	\caption{Our approach to modeling the interaction between states that affect a participant's goals and the outcome of such interaction.%
 }
 \vspace{-5mm}
	\label{fig:fig3}
\end{figure*}

%We use the linguistic concept of `aspect' and  stativise events in the discourse events  We curate stativised constructions to obtain a high quality list of causes as LLMs have been shown to be unreliable at stativizing~\cite{metheniti-etal-2022-time,friedrich-etal-2023-kind}. 
%Using the list of causes for all actions in a SAGA story and the states from the PASTA dataset~\cite{ghosh-etal-2023-pasta} we obtain annotations for alignment with a participants goal.
%Agency, volition and causal knowledge allow a participant  to achieve their goal~\cite{LILJEHOLM202178,setiya}. Knowledge of event causality allows a reader to assess a participant's progress towards the goal achievement and identify which event(s) or world state will help or hinder goal achievement. 
%\subsection{Stativization \& Causal States}
%Aspect, a linguistics concept, relates an action to a reference time\cite{friedrich-etal-2023-kind} and is useful for tasks that require semantic knowledge.  Lexical and  grammatical characteristics of events are useful to identifying states and events that can be stativised.  

%\subsection{State-Goal Alignment}

%Would knowing the state help assess achievement more accurately? Of the possible participant states in a story, some may relate (or may not) to the specific participant whose goal is being examined.  We can assume the state is directly related to the goal if the goal success changes between stories, and indirectly related or unrelated if it does not.

%1) [Complex Commonsense Reasoning] Does knowing State for a story help with inferring Goal Achievement within that story.  Can we identify whether a participant's state has an affect (direct or indirect affect) on Goal Achievement. 

%\subsection{Goal Achievement in alternative situations}
%2) [Counterfactual Reasoning] Does knowing an actual story and a counterfactual state help with inferring goal achievement in the counterfactual story, without seeing the counterfactual story context?  What happens when the state is directly related or indirectly related or unrelated?

%\subsection{Constrained story generation}
%3) [Complex Counterfactual Reasoning] Does knowing an actual story and a counterfactual state help rewrite the story such that a participant's actions in the story intend the goal.

%\subsection{Constrained Plan generation }
%4) How are plans affected by Goals?  Does state info help produce better tailored plans?

%Generalization is complicated because different sets of actions can lead to the same outcome.  Slight variations from including a new action may not change the outcome. One way to handle this is through using a \textit{state}  representation for the actions that lead to a specific goal-oriented outcome~\cite{janczyk,niv,LANGDON2019103891}.  For example, the outcome ``Tom beat his dad at ping-pong'' is highly likely to be true for all sets of actions that can be represented with the state ``Tom practiced every week'' and less likely for the actions that can be represented with the state ``Tom barely practised.''

Our \textbf{\textit{state-based Reasoning}} process is useful for several reasons: a)
context-based inferences can be nuanced and subjective and a multi-stage generalization can lead to more true outcome generalizations, b)  when the event context is unavailable or partially available, the state carries knowledge that can be used to validate the goal belief. c) provenance of the obtained context is preserved through the shared state.  However, this process is also complicated for several reasons: i) we need existing documents to use as evidence to validate the claim and there could be several documents or none!  ii) evidence in a document can be fragmented and contradictory because of changing scientific knowledge, economic indicators, political trends, etc. iii) when several evidence documents are available, their evidence quality, i.e., the mix of supporting and contradictory evidence, differs and selecting the best evidence document(s) requires lateral reasoning ~\cite{wineburg,wineburg_mcgrew}. Lateral reasoning involves critically examining several sources for associations between evidence and belief, i.e., to find agreement in information that is both explicitly stated and implied. This reasoning is complex because described situations imply information with varying certainty!~\cite{vallurupalli-etal-2022-poque}. 

Our beliefs are a combination of goal and state annotations from three implied commonsense reasoning datasets: SAGA~\cite{vallurupalli-etal-2024-saga}, UNCOMMONSENSE~\cite{zhao-etal-2024-uncommonsense} and PASTA~\cite{ghosh-etal-2023-pasta}.   While a typical claim-validation process involves searching for evidence documents, we simplify this step using a set of pre-identified documents from these datasets as evidence reports.  Like real-world evidence sources, these reports contain fragmented and contradictory evidence. We use state annotations to connect the context with the goal an identify  erroneous beliefs with a justification. We also provide a supporting hypothetical context that, if available, would make an erroneous belief truthful (shown in \cref{fig:fig2}).  %With \textit{Evidence-based Reasoning} we provides a flexible yet robust reasoning for validating unsubstantiated implicit beliefs obtained from everyday stories. 

%Based on how goal outcomes are obtained, these generalized beliefs can range from common and uncommon to erroneous!~\cite{doi:10.1073/pnas.1914085117,Wineburg2016EvaluatingIT}. 
%Like unverified claims, unverified beliefs can lead to the spread of misinformation~\cite{doi:10.1073/pnas.1912444117,vladika-matthes-2023-scientific}. Following automated claim validation~\cite{vlachos-riedel-2014-fact,schlichtkrull}, 
%Knowledge about a situation can be leveraged to guide story completion. Using SOTA LLMs, we identify implicit states a situation depends upon and use it to guide the story completion task.    For a given a set of events and a belief about what the story aims to achieve, our state-guided abductive text generation improves coherence of generated stories.  
%The progression of events in a narrative and the state changed caused by these events provide a rich set of causal interactions.  Using SOTA LLMs, we identify the implicit state changes as well as any implicit events supported by the narrative using the lexical and grammatical linguistic features of language.  Identifying counterfactual states and counterfactual events that could lead to these states, we modeled the set all events and states in a narrative as a petri-net formalism.  
%Using the code generation capabilities of Large Language Models (LLMs), we prompt models to generate states and use them to guide story completion.   Using alternate stories from the SAGA \& PASTA datasets, we curated xxx high quality actual and counterfactual events and states and their alignment with a participant's goal.  We find that prompt/chat based language models ... Llama v2.0 and Claude v2.0,    







==> sections/disclaimer.tex <==


\section*{Disclaimer}
\begin{enumerate}
\item 
\item All collected annotations were verified using random manual checks and automated filters  to ensure the annotations do not contain any risky or unsafe words, phrases or sentences. 
%\item We believe there are no risks associated with our work other than the items addressed in the limitations. 
\end{enumerate}

==> sections/inferences.tex <==
\section{Goal Knowledge based Inferences }
\label{sec:Inferences}
Goal annotations in our dataset mostly consist of implied (not stated in the story) information based on commonsense knowledge and world knowledge.  Although, we compute automated metrics listed in \cref{sec:metrics}, we mainly rely on human evaluation using the criteria in \cref{sec:def} when comparing model results.  When there is no easy baseline to compare with in our benchmarking, we compare with the GPT3.5. 

\paragraph{\textit{Goal descriptions are diverse.}}
Based on a reader's bias of the events they think as important, goal descriptions from multiple human annotators point to diverse goals in some situations.  In the collected annotations, 50\% of the story contexts lead to goal descriptions that describe slightly to vastly different goals.  Here we compare how diverse goals from models are.  

\paragraph{\textit{Overarching goals are applicable in diverse situations.}} Most of the goal descriptions are applicable to counterfactual stories.  Only 15\% of the goals are not applicable and this happens when the goals are not overarching and find other reasons.

\paragraph{\textit{State changes affect goal success.}}  A state change in an actual story leading to a counterfactual story can flip the goal success.  This happens in x\% of the situations where an unsuccessful goal is achieved with the state change and in y\% of the situations an achievable goal can no longer be achieved.  There are 2 cases leading to 4 combinations to look into:  1) where the state affects the goal  2) where the state does not affect the goal but a change in situation affects the goal  

\paragraph{\textit{Counterfactual stories do not always make sense.}}  Annotations indicate that 13\% of the stories do not make sense.  However, regardless of whether the story makes sense, human annotators are able to judge whether the goal applies to the counterfactual situation.  They are able to identify if a participant is able to achieve their goal and identify the future actions that can help achieve their goal.

\paragraph{\textit{Revising plans help with goal achievement.}} 1) Revising in actual stories and 2) revising in counterfactual stories 3) does the state have any affect on revising?




==> sections/models.tex <==
\section{Models \& Evaluation}
\label{sec:models}

\paragraph{Models:} We examine well-known open and closed chat-based large language models, GPT-4, LLaMA-3.2-8B and Mistral-7B. ...

\paragraph{Evaluation Metrics:}
\label{sec:model_eval_metrics}
We evaluate the claim label classification using the standard metric of \textbf{F1} for each of the \textit{support} \textit{refute} claim labels and a weighted average for all labels. We manually evaluate the justification and hypothetical context on whether they are each based on a reason and if the reasons for both are opposing.

generation using both automated metrics (\textbf{ROUGE}~\cite{lin-2004-rouge}, \textbf{METEOR}~\cite{lavie-agarwal-2007-meteor}, BLEU~\cite{BLEU} and BertScore~\cite{bert-score}) and a logical evaluation using both humans and GPT-4. For the Logical evaluation we examine a random sample of 100 justifications and plausible contexts (ensuring an equal number of goal and explanation constraints and plausible contexts) for explainability, coherence and cohesiveness. 





==> sections/results.tex <==
\section{Influence of Condition Category}
%\label{sec:results}

 \begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|}
 \hline
Model& \multicolumn{2}{|c|}{Direct} & \multicolumn{2}{|c|}{CoT}\\ 
& ZS & FS & ZS & FS  \\ 
\hline
FlanT5-XXL & .00/.00/.00 & .00/.00/.00 & .00/.00/.00& .00/.00/.00 \\
GPT-4o-mini& & & & \\
GPT-4o     & & & & \\
Mistral-7BI& & & & \\
Llama-8BI  & & & & \\
Llama-70BI & & & &\\
 \hline 
\end{tabular}
}
 \caption{We compare whether a pair of conditions are outcome-invariant using both a direct classification prompt and a chain-of-thought style prompt.  We report  F1 values for the 3 labels of Yes/No/Unsure to identify if a condition pair is outcome-variant.}
\label{tab:outcome-invariant}
%\vspace{-6mm}
\end{table}





\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
Model& \multicolumn{2}{|c|}{Full Context}  & \multicolumn{2}{|c|}{Partial Context}  & \multicolumn{2}{|c|}{Goal Intent}  & State\\ 
& nS & wS& nS & wS& nS & wS& Only \\ 
\hline
FlanT5-XXL  & .85/.85/.44& .59/.49/.10 &.70/.77/.16 &.55/.61/.03 & .61/.64/.05& .72/.64/.05&.57/.75/.07\\
%FlanT5-XXL (FS) &.57/.69/.00 & .57/.03/.02& .59/.70/.00&.54/.47/.02 & .56/.69/.00& .61/.34/.00&.60/.69/.13\\
GPT-4o-mini  & .85/.86/.29 & .60/.59/.09& .68/.78/.16& .58/.48/.05& .41/.61/.10& .71/.61/.01&.55/.53/.05\\
%GPT-4o-mini (FS)& &  &&&&&&\\
GPT-4o &.83/.88/.33 & .61/.61/.14& .45/.76/.13& .46/.46/.07 & .03/.64/.09& .44/.31.06 &.09/.17/.05\\
%GPT-4o (FS)     &  &&&&&&\\
Mistral-7BI& .79/.79/.28& .55/.55/.09& .69/.64/.14& .45/.48/.04& .54/.62/.12& .54/.59/.06&.44/.64/.04\\
%Mistral-7BI (FS)& .25/.48/.15 & .26/.05/.05& .33/.50/.12& .34/.28/.04& .32/.58/.10& .24/.19/.05&.26/.17/.04\\
Llama-8BI   & .81/.82/.00& .57/.61/.00& .71/.72/.00& .53/.66/.00& .52/.53/.00& .70/.72/.00&.60/.70/.02\\
%Llama-8BI (FS)& .42/.72/.07& .24/.26/.05& .30/.65/.09& .19/.28/.05& .31/.63/.05& .32/.30/.05&.24/.30/.05\\
Llama-70BI & .84/.83/.32 &.56/.63/.06& .71/.79/.15& .51/.62/.05& .37/.40/.02& .59/.67/.03& .47/.54/.05\\
%Llama-70BI (FS) & .58/.77/.12& .37/.40/.05& .48/.75/.10& .28/.32/.05& .20/.62/.10& .25/.36/.05& .19/.37/.04\\
\hline 
\end{tabular}
}
 \caption{Only opposing Multi-label classification of Outcomes being True, False or Unsure.  Reported Accuracy/F1 for True and False for condition along with full, partial, goal and no context and compared it with a baseline of full context without any condition.  }
\label{tab:variant-condition-outcome-labeling}
%\vspace{-6mm}
\end{table}


\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
Model& \multicolumn{2}{|c|}{Full Context}  & \multicolumn{2}{|c|}{Partial Context}  & \multicolumn{2}{|c|}{Goal Intent}  & State\\ 
& nS & wS& nS & wS& nS & wS& Only \\ 
\hline
FlanT5-XXL  & .80/.81/.19& .57/.47/.04 &.62/.73/.17 &.50/.57/.06 & .62/.69/.03& .64/.54/.07&.47/.66/.13\\
%FlanT5-XXL (FS) &.40/.72/.20 & .29/.08/.10& .20/.71/.20&.35/.24/.10 & .55/.70/.13& .47/.29/.10&.48/.48/.12\\
GPT-4o-mini  & .80/.83/.24 & .57/.54/.11& .62/.77/.21& .54/.41/.10& .44/.65/.13& .62/.49/.08&.46/.41/.11\\
%GPT-4o-mini (FS)& &  &&&&&&\\
GPT-4o &.80/.86/.47 & .58/.56/.22& .37/.77/.23& .40/.36/.13 & .05/.69/.19& .36/.23/.11 &.08/.11/.10\\
%GPT-4o (FS)     &  &&&&&&\\
Mistral-7BI& .74/.75/.11& .52/.52/.10& .59/.67/.17& .38/.40/.10& .57/.69/.18& .46/.50/.13&.35/.58/.11\\
%Mistral-7BI (FS)&.33/.48/.16& .29/.41/.10& .36/.50/.17& .38/.37/.10& .32/.57/.19& .26/.29/.09&.26/.33/.09\\
Llama-8BI   & .77/.76/.00& .53/.59/.02& .63/.61/.04& .44/.63/.02& .58/.63/.01& .57/.62/.10& .44/.63/.04\\
%Llama-8BI (FS)& .33/.48/.16& .29/.41/.10& .36/.50/.17& .38/.37/.10& .32/.57/.19& .26/.29/.09&.26/.33/.09\\
Llama-70BI & .78/.77/.20 &.55/.61/.12& .64/.73/.20& .46/.57/.11& .35/.38/.02& .48/.57/.11& .49/.43/.11\\
%Llama-70BI (FS) & .81/.84/.35& .61/.62/.17& .63/.79/.25& .47/.47/.12& .31/.65/.17& .38/.38/.11& .27/.37/.10\\
\hline 
\end{tabular}
}
 \caption{Only opposing Multi-label classification of Outcomes being True, False or Unsure.  Reported Accuracy/F1 for True and False for condition along with full, partial, goal and no context and compared it with a baseline of full context without any condition.  }
\label{tab:variant-condition-outcome-labeling}
%\vspace{-6mm}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|}
 \hline
Model& \multicolumn{2}{|c|}{Full Context}  & \multicolumn{2}{|c|}{Partial Context}  & \multicolumn{2}{|c|}{Goal Intent}  & State\\ 
& nS & wS& nS & wS& nS & wS& Only \\ 
\hline
T5-11b (FS)& & & & & & &\\
FlanT5-XXL (ZS) & .88/.75/.24& .87/.76/.02&.63/.68/.16 &.75/.67/.08 & .77/.07/.06 & .76/.57/.08&.46/.57/.19\\
FlanT5-XXL (FS) &.77/.00/.05 & .76/.04/.04& .76/.15/.00&.74/.47/.02 & .77/.05/.04 & .75/.32/.02&.54/.52/.15\\
GPT-4o-mini (ZS)&.83/.73 & .84/.73& .65/.50& 76/.56 & .50/.33 & .71/.50&.45/.42\\
GPT-4o-mini (FS)& .72/.71& .66/.68& .51/.66& .61/.30& .43/.45 & .27/.57&.09/.58\\
GPT-4o (ZS)& & & & & & &\\
GPT-4o (FS)     & .47/.50& .50/.45& .41/.45& .30/.40& .07/.24 & .24/.35&.06/.16\\
Mistral-7BI (ZS)& .41/.11& .21/.34& .41/.26& .44/.40& .56/.16 & .56/.23&.51/.35\\
Mistral-7BI (FS)& & & & & & &\\
Llama-8BI (ZS)  & .81/.73& .80/.73& .69/.63& .64/.65& .61/.47 & .67/.60&.58/.62\\
Llama-8BI (FS)  & .81/.76& .82/.75& .58/.65& .62/.64& .70/.29 & .70/.60&.52/.61\\
Llama-70BI (ZS) & & & & & & &\\
Llama-70BI (FS) & & & & & & &\\
\hline 
\end{tabular}
}
 \caption{Multi-label classification of Outcomes being True, False or Unsure.  Reported Accuracy/F1 for True and False for condition along with full, partial, goal and no context and compared it with a baseline of full context without any condition.  }
\label{tab:invariant-condition-outcome-labeling}
%\vspace{-6mm}
\end{table}

\section{Influence of Condition Category}
%\label{sec:results}
\section{Cross-Domain Application to News Stories }



\begin{figure}[t]
    \centering  
    \begin{subfigure}[b]{0.48\columnwidth}
    \includegraphics[trim=0in 0in 0in 0in, scale=.48]{test.pdf}
    \caption{\label{fig:fig3a}  }
    \end{subfigure}
    ~
    %\hfill
    \begin{subfigure}[b]{0.4832\columnwidth}
    \includegraphics[trim=0in 0in 0in 0in, scale=.48]{  test.pdf}
    \caption{\label{fig:fig3b} }
    \end{subfigure}

    \caption{Outcome validation through condition-based reasoning.  Our research questions leverage PASTA~\cite{ghosh-etal-2023-pasta} and SAGA~\cite{vallurupalli-etal-2024-saga} datasets to validate story outcomes. We generate outcomes from SAGA goals and generate PASTA style conditions. We validate these outcomes, using both generated conditions and the crowd annotated conditions from PASTA.}
    \label{fig:fig3}
 \vspace{-3mm}
\end{figure}

%--------------------------------------------
\begin{figure*}[t] 
    \centering  
    \begin{subfigure}[b]{0.49\textwidth}
    \vspace{-3mm}
    \includegraphics[trim=0in 0in 0in 0in, scale=.46]{sections/figures/Fig3a-invariant.pdf}
    \vspace{-10mm}
    \caption{\label{fig:fig3a} Outcome identification with \textbf{invariant condition} pairs. }
    \end{subfigure}
    ~
    \begin{subfigure}[b]{0.49\textwidth}
    \vspace{-3mm}
    \includegraphics[trim=0in 0in 0in 0in, scale=.46]{sections/figures/Fig3b-variant.pdf}
    \vspace{-10mm}
    \caption{\label{fig:fig3b} Outcome identification with \textbf{variant condition} pairs.}
    \end{subfigure}
    \vspace{-6mm}
    \caption{Identifying Outcome labels using varying amounts of context consisting of a SAGA story and a PASTA crowd annotated condition supported by the story.} %The conditions used include the crowd annotated (from PASTA) and generated conditions. (legend for the 6 models compared is on the right for all three graphs.)}
    \label{fig:fig3}
 %\vspace{-6mm}
\end{figure*}

\textbf{A:} Jared was tossing and turning all night. He kept hearing a buzz right next to his ear. Every time he tried to swat, the sound went away. As he was drifting off, something landed right on his large nose. He hit it and discovered that it was a now dead fly! \newpage
\textbf{B:} Jared is a light sleeper. \newpage 
\textbf{C:} Jared slept peacefully. \newpage
For the context in A and the condition in B, Is the statement in C true? \newpage Please indicate with a 'Y' for yes, 'N' for no and 'U' for unsure. Do not give an explanation. 
&
\\
\hline\hline




 

==> sections/unused_results.tex <==

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.79&.44&.80&.30 \\ 
& T511b  &.50&.29&.58&.31 \\
& fT5b   &.59&.31&.64&.34 \\
& fT5l   &.26&.24&.61&.33 \\
& fT5xl  &.29&.27&.29&.19 \\
& fT5xxl &.29&.27&.42&.26 \\
& gpt3.5t&.57&.53+&.65&.38+ \\
& gpt4   &.64&.59+&.79&.42+ \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.62&.26&.62&.26 \\ 
& T511b  &.48&.31&.52&.34 \\
& fT5b   &.49&.30&.47&.28 \\
& fT5l   &.45&.31&.43&.28 \\
& fT5xl  &.40&.28&.44&.30 \\
& fT5xxl &.42&.28&.43&.29 \\
& gpt3.5t&.31&.22&.48&.31+ \\
& gpt4   &.44&.30+&.59&.38+ \\
\hline
\end{tabular}
}
 \caption{Identifying whether a revision will help with goal achievement.  }
\label{tab:goals-revision-metrics}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.79&.44&.53&.55 \\ 
& T511b  &.52&.50&.52&.52 \\
& fT5b   &.47&.32&.43&.30 \\
& fT5l   &.67&.40&.59&.59 \\
& fT5xl  &.79&.44&.52&.42 \\
& fT5xxl &.71&.42&.56&.53 \\
& gpt3.5t&.64&.52&.67&.65 \\
& gpt4   &.64&.52&.51&.50 \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.56&.36&.61&.38 \\ 
& T511b  &.53&.53&.54&.54 \\
& fT5b   &.39&.28&.41&.29 \\
& fT5l   &.51&.49&.61&.61 \\
& fT5xl  &.59&.43&.47&.42 \\
& fT5xxl &.60&.50&.53&.51 \\
& gpt3.5t&.53&.49&.58&.57+ \\
& gpt4   &.53&.47&.60&.60+ \\
\hline
\end{tabular}
}
 \caption{Identifying whether achievable goals are revised.}
\label{tab:achievable-goals-revised-metrics}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.79&.44&.80&.45 \\ 
& T511b  &.20&.16&.20&.17 \\
& fT5b   &.79&.44&.59&.42 \\
& fT5l   &.57&.36&.71&.42 \\
& fT5xl  &.79&.44&.80&.45 \\
& fT5xxl &.79&.44&.80&.45 \\
& gpt3.5t&.79&.44&.80&.45 \\
& gpt4   &&&& \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.62&.38&.62&.38 \\ 
& T511b  &.38&.28&.20&.17 \\
& fT5b   &.79&.47&.63&.40 \\
& fT5l   &.56&.67&.60&.50 \\
& fT5xl  &.62&.38&.62&.38 \\
& fT5xxl &.62&.38&.62&.38 \\
& gpt3.5t&.62&.38&.62&.38 \\
& gpt4   &&&& \\
\hline
\end{tabular}
}
 \caption{Identifying Original vs Revised plans by Models }
\label{tab:plan-revision}
\end{table}


\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
 \hline
& \multicolumn{4}{|c|}{Overall Satisfaction} & \multicolumn{4}{|c|}{ Achievement Satisfac.}\\  &\multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterfac.}&\multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterfac.}\\ 
Model&Acc&mF1&Acc&mF1&Acc&F1&Acc&F1\\
\hline
Maj.   &.72&.28&.62&.26&.87&.47&.62&.26\\ 
T511b  &.60&.33&.52&.32&.53&.43&.52&.48  \\
fT5b   &.74&.36&.64&.36   &.89&.67&.73&.54 \\
fT5xxl &.87&.58&.66&.45&.89&.77&.68&.65\\
gpt3.5t&.84&.54&.63&.48&.86&.75&.64&.62 \\
gpt4   &.87&.57&.67&.50&.89&.78&.70&.66 \\
\hline
\end{tabular}
}
\caption{Participant's satisfaction with the state of goal achievement}
\label{tab:goal-satisfaction-metrics}
\end{table}

\begin{table}[t]
\centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} 
& Maj.   &.89&.47&.78&.44 \\ 
& T511b  &.57&.44&.52&.47 \\
& fT5b   &.88&.59&.73&.45 \\
& fT5l   &.86&.74&.68&.64 \\
& fT5xl  &.88&.68&.81&.75 \\
& fT5xxl &.92&.82&.82&.79 \\
& gpt3.5t&.85&.73&.73&.70 \\
& gpt4   &.88&.72&.82&.78 \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.   &.87&.47&.62&.26 \\ 
& T511b  &.53&.43&.52&.48 \\
& fT5b   &.89&.67&.73&.54 \\
& fT5l   &.81&.70&.59&.57 \\
& fT5xl  &.92&.82&.70&.65 \\
& fT5xxl &.89&.77&.68&.65 \\
& gpt3.5t&.86&.75&.64&.62 \\
& gpt4   &.89&.78&.70&.66 \\
\hline
\end{tabular}
}
\caption{Participant's satisfaction measurement for achievable goals}
\label{tab:goal-satisfaction-with-achievement-metrics}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|l|c|c|c|c|}
 \hline
&& \multicolumn{2}{|c|}{Actual} & \multicolumn{2}{|c|}{Counterf.}\\ 
Split&Model&Acc&mF1&Acc&mF1\\
\hline
\multirow{5}{*}{Val} &
Maj.   &.73&.28&.58&.24 &.62&.38&.48&.22\\ 
 T511b  &.68&.39&.65&.42 &.66&.38&.62&.35\\
 fT5b   &.72&.28&.61&.32 &.59&.42&.54&.32 \\
 fT5xxl &.67&.41&.85&.59 &.75&.47&.80&.55\\
 gpt3.5t&.64&.40&.80&.55 &.67&.42&.74&.54 \\
 gpt4   &.58&.37&.65&.46 &.80&.68&.80&.68\\
 \hline
 T5b-ft &.65&.41&.73&.50 &.72&.42&.70&.49\\
 fT5b-ft&.65&.37&.77&.53 &.74&.44&.72&.50\\
 \hline
 & Maj.    &.73&.28&.58&.24 \\ 
& T511b   &.68&.39&.65&.42 \\
& T5b-ft  &.65&.41&.72&.49 \\
& fT5b    &.72&.28&.61&.32 \\
& fT5b-ft &.65&.37&.77&.53 \\
& fT5l    &.66&.39&.77&.53 \\
& fT5l-ft &.67&.38&.82&.57 \\
& fT5xl   &.64&.39&.82&.57 \\
& fT5xl-ft&.71&.47&.78&.58 \\
& fT5xxl  &.67&.41&.85&.59 \\
& gpt3.5t &.64&.40&.80&.55 \\
& gpt4    &.58&.37&.65&.46 \\
 \hline
\hline
\multirow{5}{*}{Test} 
& Maj.    &.62&.38&.48&.22 \\ 
& T511b   &.66&.38&.62&.35 \\
& T5b-ft  &.72&.42&.72&.49 \\
& fT5b    &.59&.42&.54&.32 \\
& fT5b-ft &.74&.44&.72&.50 \\
& fT5l    &.66&.57&.70&.49 \\
& fT5l-ft &.74&.45&.73&.54 \\
& fT5xl   &.73&.46&.79&.55 \\
& fT5xl-ft&.76&.49&.71&.55 \\
& fT5xxl  &.75&.47&.80&.55 \\
& gpt3.5t &.67&.42&.74&.54 \\
& gpt4    &.80&.68&.80&.68 \\
\hline
\end{tabular}
}
 \caption{Model identification of Goal achievement at the end of a story.  }
\label{tab:all-goals-success-in-story-metrics}
\end{table}
\emph{\textbf{Are larger models better at identifying  participants' satisfaction?}}
A proxy for goal achievement is a participant's satisfaction during and after goal achievement.  We cast identifying satisfaction as an entailment task with the story, goal and next action as premise and ask if the participant is satisfied with their goal achievement with the choices of Yes, No and Unsure.  Since participants may not always be satisfied with achieved goals, or unsatisfied with unachieved goals as mentioned in \cref{sec:prospective-goal-knowledge} we repeat this task with only achieved goals and cast it as a binary inference.  Refer to \cref{tab:task-prompts} for the prompt setup for both variations of the task. The results from this variation are presented in \cref{tab:goal-satisfaction-with-achievement-metrics}.  Performance for both the setups improves with model size. FlanT5's fine-training on a large number of tasks helps on this task as even the base Flan-T5 model performs better than T5-11b. All models perform better for the actual story context than the counterfactual story context.  We attribute this difference to the fact that a goal annotated for an actual story may not perfectly suit the counterfactual story context. 

\begin{table}[t]
 \centering
\resizebox{.68\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|}
 \hline
Model& Goal (F1)& Full Agr. (F1) & Partial A. (F1)\\ 
\hline
Maj.  &.68&.67&.00 \\
%Ref.   &   &.  &.  &.  \\
%T511b   &.47/.36&.47/.26&.52/.38\\
fT5b (0 \& 3-shot)&.51/.60&.55/.62&.48/.59 \\
%ft5l    &.54/.65&.60/.70&.49/.62\\
%ft5xl   &.62/.47&.67/.57&.58/.38\\
fT5xxl (0 \& 3-shot)&.76/.73&.90/.90&.66/.58 \\
gpt3.5t (0-shot)&.63/.56&.78/.76&.53/.39\\
gpt3.5t (3-shot)&.69/.65&.79/.79&.61/.52\\
gpt4  (0-shot)&.76/.72 &.87/.86 &.67/.52 \\
gpt4  (3-shot)&.76/.72&.88/.88&.66/.48\\
\hline
T5b-ft (0-shot)&.58/.69&.63/.72&.54/.66 \\%(epoch 4) 
fT5b-ft (0-shot)&.56/.69&.63/.73&.51/.65 \\%(epoch 1)
fT5b-ft (3-shot)&\textbf{.75/.79}&.85/.87&\textbf{.65/.69}\\%(epoch 1)
\hline
\end{tabular}
}
 \caption{Evaluation of goal transferability comparing performance in full \& partial agreement stories.  %Significantly higher (compared to all other models) are bolded.
 %\todo[inline]{check stat. sign.}
% \todo[inline]{limiting verbosity, state one sentence take-away}
}
\label{tab:counterfactual-applicability-metrics}
\vspace{-5mm}
\end{table}

\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
 \hline
 & \multicolumn{5}{|c|}{Actual Story} & \multicolumn{5}{|c|}{Counterfactual Story}\\  Model  & Rou  & ME&P.Type&\multicolumn{2}{|c|}{Human Eval.} & Rou &ME&P.Type&\multicolumn{2}{|c|}{Human Eval.}\\ 
  Type&  L &TR &Acc/F1& Plan &Type&  L &TR&Acc/F1& Plan &Type\\
 \hline
\hline
Ref/Maj    &-&-&.62/.77&4.28&4.28&-&-&.62/.77&4.31&4.29 \\ 
%&&Ref    &&&&&4.25&3.95 &&&&&4.34&4.34\\
fT5b (3-shot)&.19&.24&.47/.37 &\underline{3.5}&\underline{3.21} &.20&.24&.55/.48&\underline{3.09}&\underline{2.85} \\
%&&Ref    &&&&&4.20&4.20 &&&&&4.23&4.23\\
fT5xxl (3-shot)&.22&.24&.52/.44&\underline{3.26}&\underline{2.78}&.20&.23&.52/.38&\underline{3.57}&\underline{2.96}\\
%&&Ref    &&&&4.29&4.29&  &&&&&4.39&4.36\\
gpt3.5t (3-shot)&.19&.25&.75/.83&3.87&\underline{2.35}&.17&.23&.65/.72&3.99&\underline{2.87}\\
%&&Ref    &&&&&4.29&4.23 &&&&&4.37&4.37 \\
gpt4 (3-shot) &.20&.21&.78/.82&4.16&\underline{3.22}&.17&.20&.75/.79&4.07&\underline{2.95}\\
\hline
%%T5b-ft (0-shot) &.16&.11&.70/.78&3.60&\underline{3.16}&.12&.10&.76/.83&4.1&\underline{3.33}\\
fT5b-ft (0-shot)&.16&.10&.72/.79&4.07&\underline{3.15}&.12&.09&.89/.91&3.72&\underline{3.33}\\ 
fT5b-ft (3-shot)&.14&.17&.72/.79&\underline{2.96}&\underline{2.89}&.10&.09&.89/.91&\underline{2.78}&\underline{2.99}\\ 
%fT5l-ft&.16&.12&.75/.82&-&-&.15&.11&.86/.89&-&-\\
\hline
\end{tabular}
}
 \caption{Evaluation of model generated plans and plan types.  Ref/Maj is the majority class accuracy/F1 for the Plan Type and gold label human evaluation scores. Underlined scores are significantly lower than reference. 
%\todo[inline]{work on narrative}
}
\label{tab:future-plan-manual-metrics}
\vspace{-2mm}
\end{table}
\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
 \hline
 & \multicolumn{5}{|c|}{Actual Story} & \multicolumn{5}{|c|}{Counterfactual Story}\\  Model  & Rou  & ME&P.Type&\multicolumn{2}{|c|}{Human Eval.} & Rou &ME&P.Type&\multicolumn{2}{|c|}{Human Eval.}\\ 
  Type&  L &TR &F1& Plan &Type&  L &TR&F1& Plan &Type\\
 \hline
\hline
Ref/Maj    &-&-&.77&4.28&4.28&-&-&.77&4.31&4.29 \\ 
%&&Ref    &&&&&4.25&3.95 &&&&&4.34&4.34\\
fT5b (3-shot)&.19&.24&.37 &\underline{3.5}&\underline{3.21} &.20&.24&.48&\underline{3.09}&\underline{2.85} \\
%&&Ref    &&&&&4.20&4.20 &&&&&4.23&4.23\\
fT5xxl (3-shot)&.22&.24&.44&\underline{3.26}&\underline{2.78}&.20&.23&.38&\underline{3.57}&\underline{2.96}\\
%&&Ref    &&&&4.29&4.29&  &&&&&4.39&4.36\\
gpt3.5t (3-shot)&.19&.25&.83&3.87&\underline{2.35}&.17&.23&.72&3.99&\underline{2.87}\\
%&&Ref    &&&&&4.29&4.23 &&&&&4.37&4.37 \\
gpt4 (3-shot) &.20&.21&.82&4.16&\underline{3.22}&.17&.20&.79&4.07&\underline{2.95}\\
%\hline
%%T5b-ft (0-shot) &.16&.11&.70/.78&3.60&\underline{3.16}&.12&.10&.76/.83&4.1&\underline{3.33}\\
fT5b-ft (0-shot)&.16&.10&.79&4.07&\underline{3.15}&.12&.09&.91&3.72&\underline{3.33}\\ 
%fT5b-ft (3-shot)&.14&.17&.79&\underline{2.96}&\underline{2.89}&.10&.09&.91&\underline{2.78}&\underline{2.99}\\ 
%fT5l-ft&.16&.12&.75/.82&-&-&.15&.11&.86/.89&-&-\\
\hline
\end{tabular}
}
 \caption{Evaluation of model generated plans and plan types.  Ref/Maj is the majority class F1 for Plan Type and gold label human evaluation scores. Underlined scores are significantly lower than reference. Human evaluation examines the correctness of plan and its type.
%\todo[inline]{work on narrative}
}
\label{tab:future-plan-manual-metrics}
\vspace{-2mm}
\end{table}

\begin{table*}[t]
\centering
\resizebox{.98\textwidth}{!}{
 \begin{tabular}{l|l|c|c|c|c|c|c|c|c|c|c|c|c|}
 \cline{2-14}
  &  & \multicolumn{3}{|c|}{Rouge} & MET- & \multicolumn{2}{|c|}{BLEU} & Bert-&\multicolumn{5}{|c|}{Human Evaluation}\\ 
  & & R1 & R2 & RL & EOR & Corpus & Google & Score&Cohere &Explain & Faith & Truth & Intent\\
 \cline{2-14}
 \cline{2-14}
 &Reference & \multicolumn{7}{|c|}{-} &4.76 & 4.67 & 4.9 & 4.91 & 4.74 \\ 
 \cline{2-14}
\multirow{6}{*}{Val Split} 
& T5-11b  &  &  &  &  &  &  & &&&&& \\
& flanT5b  &  .37  &  .14 & .36 & .34  &  0.9 & .14 &.86& 3.72- & 3.94- &4.15-&3.79- & 3.64-  \\
& flanT5l  & .41  & .22  & .4 & .3  & .16  & .14 & .84 &&&&&\\
& flanT5xl & .42  & .21 & .4 & .33  & .17  & .15 & .85&&&&&\\
& flanT5xxl&  .45 & .25 & .44 & .43  & .2  & .2 & .86 &4.5&4.37&4.86&4.92 &4.38\\
& gpt3.5t  &  .44 & .21 & .42 &  .49 & .11  & .15 & &4.68&\textbf{4.93+}&4.86&4.86&4.42\\
& gpt4     & .5  & .3 & .49 &.51   &.21   & .23 & &4.94&4.9&4.98&4.98&4.86\\
\hline
\multirow{10}{*}{Act.}&\multirow{5}{*}{Val}
 &\multicolumn{3}{|l|}{Ref mean vals (var < \%) }&4.81&4.78 &4.91 &4.97 &4.82 \\ 
&& Ref    &&      &4.73 &4.76 &4.96 &5.00 &4.84 \\
&&fT5b    &.38&.36&\underline{3.61}&\underline{3.85}&\underline{4.20}&\underline{3.69}&\underline{3.52} \\ 
&& Ref    &&      &4.83 &4.79 &4.84 &4.92 &4.75 \\
&& fT5xxl &.44&.44&4.47 &4.43 &4.93 &4.92 &4.37 \\
&& Ref    &&      &4.75 &4.68 &4.87 &5.00 &4.69 \\
&& gpt3.5t&.43&.50&4.67 &\textbf{4.96}&4.84 &4.84 &4.53 \\
&& Ref    &&      &4.92 &4.88 &4.96 &4.96 &4.83 \\
&& gpt4   &.48&.53&4.91 &4.87 &5.00 &5.00 &4.8\\
\cline{2-10}
&\multirow{5}{*}{Test} 
 &\multicolumn{3}{|l|}{Ref mean vals (var < \%) }&4.74&4.69&4.78&4.78&4.49 \\ 
&& Ref    &&      &4.73 &4.67 &4.78 &4.85 &4.43 \\
&& fT5b   &.42&.40&\underline{3.95}&\underline{4.19}&4.50 &\underline{4.35}&\underline{3.72} \\
&& Ref    &&      &4.75 &4.71 &4.77 &4.88 &4.54 \\
&& fT5xxl &.50&.49&4.49 &4.65 &4.83 &4.81 &\underline{4.03} \\
&& Ref    &&      &4.73 &4.65 &4.76 &4.74 &4.49 \\
&& gpt3.5t&.44&.52&4.53 &4.59 &\textbf{4.95}&\underline{3.89}&4.90 \\
&& Ref    &&      &4.75 &4.71 &4.81 &4.81 &4.48 \\
&& gpt4   &.53&.55&\underline{4.46}&4.44 &4.82 &4.82 &\underline{3.92}\\
\hline
\hline
  &Reference & \multicolumn{7}{|c|}{-} &4.74 & 4.73 & 4.79 & 4.83 & 4.57 \\ 
\hline
\multirow{6}{*}{Test Split} 
& T5-11b  &  &  &  &  &  &  & &&&&& \\
& flanT5b & .44 & .21 & .42 & .4 & .11 & .16 & .86 &3.47-&3.78-&4.1-&3.97-&3.32-\\
& flanT5l &.45 & .23 & .45 & .32 & .18 & .15 & .86 &&&&&\\
& flanT5xl  & .47 & .25 & .46 & .36  & .18 & .16 & .86 &&&&&\\
& flanT5xxl  & .50 & .27  & .49 & .46  & .2  & .2 & .86&4.31-&4.47- &4.67&4.71&4.0-\\
& GPT3.5t & .44 & .22 & .42 &  .49&  .1 & .14&&4.47-&4.47-&4.86&4.81&3.9-\\
& GPT4  & .52 & .32 & .51 & .53 & .22 & .24 &  &4.53&4.49&4.81&4.82&4.00-\\
 \hline
 \cline{2-9}
 \end{tabular}
 }
 \caption{Automated and Human Evaluation scores for model generated Goals.\todo[inline]{fix table} }
\label{tab:goal-description-all-metrics}
\end{table*}


\begin{table}[t]
 \centering
\resizebox{.98\columnwidth}{!}{
 \begin{tabular}{|l||l|l|c|c|c|c|c|}
 \hline
  Story &Split&Model  & Rouge & MET &\multicolumn{3}{|c|}{Human Eval}\\ 
  Type& & & L & EOR & Cohere &Cohesive & Explain \\
 \hline
\hline
\multirow{10}{*}{Act.}&\multirow{5}{*}{Val}
 &Ref & &&4.70&4.64&4.79 \\ 
&&Ref     & &&4.53&4.58&4.5 \\ 
&& fT5b   &.29&.29&\underline{2.06}&\underline{1.64} &\underline{1.17}\\
&&Ref     & &&4.85&4.77&4.92 \\ 
&& fT5xxl &.45&.49&4.77&4.49&\underline{4.24}\\
&&Ref     & &&4.72&4.60&4.88 \\ 
&& gpt3.5t&.40&.46&4.72&4.75&4.88\\
&&Ref     & &&4.68&4.60&4.84 \\ 
&& gpt4   &.45&.48&4.92&\textbf{4.88}&4.96\\
\cline{2-8}
&\multirow{5}{*}{Test} 
 &Ref     &  &&4.68&4.53&4.88 \\ 
&&Ref     & &&4.67&4.58&4.91 \\ 
 && fT5b  &.30&.31 &\underline{2.35}& \underline{2.15} & \underline{1.39}\\
&&Ref     & &&4.58&4.44&4.84 \\ 
&& fT5xxl &.47&.50&4.62&4.54&\underline{3.97}\\
&&Ref     & &&4.77&4.63&4.88 \\ 
&& gpt3.5t&.43&.48&4.85&4.71&4.83\\
&&Ref     & &&4.68&4.49&4.90 \\ 
&& gpt4   &.45&.50&4.87&4.75&4.87\\
\hline
\hline
\multirow{10}{*}{Cou.}&\multirow{5}{*}{Val}
 &Ref     & &&4.55&4.54&4.85 \\ 
&&Ref     & &&4.47&4.59&4.77 \\ 
&& fT5b   &.30&.30&\underline{1.73}&\underline{1.76}&\underline{1.43}\\
&&Ref     & &&4.60&4.40&4.67 \\ 
&& fT5xxl &.45&.49&4.77&4.45&\underline{4.16}\\
&&Ref     & &&4.56&4.52&4.83 \\ 
&& gpt3.5t&.40&.46&\textbf{4.93}&\textbf{4.84}&4.88\\
&&Ref     & &&4.67&4.59&4.83 \\ 
&& gpt4   &.44&.48&4.88&4.88&4.88\\
\cline{2-8}
&\multirow{5}{*}{Test} 
 &Ref     & &&4.71&4.60&4.61 \\ 
&&Ref     & &&4.70&4.55&4.50 \\ 
&& fT5b   &.31&.31&\underline{1.87}&\underline{2.00}&\underline{1.56}\\
&&Ref     & &&4.75&4.55&4.63 \\ 
&& fT5xxl &.47&.49&\underline{3.92}&\underline{3.83}&\underline{3.69}\\
&&Ref     & &&4.79&4.67&4.65 \\ 
&& gpt3.5t&.41&.47&4.79&4.62&4.82\\
&&Ref     & &&4.79&4.63&4.65 \\ 
&& gpt4   &.45&.49&4.63&4.57&\textbf{4.95}\\
\hline
\end{tabular}
}
 \caption{Automated and Human Evaluation scores for model generated Next Actions. \todo[inline]{fix table} }
\label{tab:next-actions-manual-metrics2}
\end{table}

